Term Graph Representations for Cyclic Lambda-Terms

We study various representations for cyclic lambda-terms as higher-order or as first-order term graphs. We focus on the relation between `lambda-higher-order term graphs' (lambda-ho-term-graphs), which are first-order term graphs endowed with a well-behaved scope function, and their representations as `lambda-term-graphs', which are plain first-order term graphs with scope-delimiter vertices that meet certain scoping requirements. Specifically we tackle the question: Which class of first-order term graphs admits a faithful embedding of lambda-ho-term-graphs in the sense that: (i) the homomorphism-based sharing-order on lambda-ho-term-graphs is preserved and reflected, and (ii) the image of the embedding corresponds closely to a natural class (of lambda-term-graphs) that is closed under homomorphism? We systematically examine whether a number of classes of lambda-term-graphs have this property, and we find a particular class of lambda-term-graphs that satisfies this criterion. Term graphs of this class are built from application, abstraction, variable, and scope-delimiter vertices, and have the characteristic feature that the latter two kinds of vertices have back-links to the corresponding abstraction. This result puts a handle on the concept of subterm sharing for higher-order term graphs, both theoretically and algorithmically: We obtain an easily implementable method for obtaining the maximally shared form of lambda-ho-term-graphs. Also, we open up the possibility to pull back properties from first-order term graphs to lambda-ho-term-graphs. In fact we prove this for the property of the sharing-order successors of a given term graph to be a complete lattice with respect to the sharing order. This report extends the paper with the same title (http://arxiv.org/abs/1302.6338v1) in the proceedings of the workshop TERMGRAPH 2013.

==> figs/pstricks/Makefile <==
# create a picture for each file containing a Lagtx fragment in the directory

# disable implicit rules
.SUFFIXES:

TEXFILES=$(wildcard *.tex)

#noflags:
#	make -r default

default: pdfs

#pdfs: $(TEXFILES:.tex=.lgr.pdf) $(TEXFILES:.tex=.sgr.pdf) $(TEXFILES:.tex=.ltg-u.pdf) $(TEXFILES:.tex=.ltg-l.pdf) $(TEXFILES:.tex=.ltg-u-bl.pdf) $(TEXFILES:.tex=.ltg-l-bl.pdf)
pdfs: $(TEXFILES:.tex=.lgr.pdf)

%.lgr.gtx: %.tex
	cat mk/prelude.tex > $@
	echo '\\input{macros/lambdagraph}' >> $@
	cat $< >> $@
	cat mk/postlude.tex >> $@

#%.sgr.gtx: %.tex
#	cat mk/prelude.tex > $@
#	echo '\\input{macros/scopedgraph}' >> $@
#	cat $< >> $@
#	cat mk/postlude.tex >> $@

#%.ltg-u-bl.gtx: %.tex
#	cat mk/prelude.tex > $@
#	echo '\\input{macros/ltg-bl}' >> $@
#	echo '\\newcommand\\nlabel[1]{}' >> $@
#	cat $< >> $@
#	cat mk/postlude.tex >> $@
#
#%.ltg-l-bl.gtx: %.tex
#	cat mk/prelude.tex > $@
#	echo '\\input{macros/ltg-bl}' >> $@
#	echo '\\newcommand\\nlabel[1]{#1}' >> $@
#	cat $< >> $@
#	cat mk/postlude.tex >> $@
#
#%.ltg-u.gtx: %.tex
#	cat mk/prelude.tex > $@
#	echo '\\input{macros/ltg}' >> $@
#	echo '\\newcommand\\nlabel[1]{}' >> $@
#	cat $< >> $@
#	cat mk/postlude.tex >> $@
#
#%.ltg-l.gtx: %.tex
#	cat mk/prelude.tex > $@
#	echo '\\input{macros/ltg}' >> $@
#	echo '\\newcommand\\nlabel[1]{#1}' >> $@
#	cat $< >> $@
#	cat mk/postlude.tex >> $@

include mk/figure.mk


==> figs/pstricks/lambdatgs_not_closed_under_funbisim_convfunbisim_item_i.tex <==
\lgr{
\app{\abs\var}{\abs\var}
}


==> figs/pstricks/lambdatgs_not_closed_under_funbisim_convfunbisim_item_ii.tex <==
\lgr{
\app{\abs\var}{\abs{\nil}}
}


==> figs/pstricks/lambdatgs_not_closed_under_funbisim_convfunbisim_item_iii.tex <==
\lgr
{
\abs{\app{\abs{\s{\var}}}{\abs{\s{\var}}}}
}


==> figs/pstricks/lambdatgs_over_siglambda12_not_closed_under_funcbisim.tex <==
\lgr
{
\app{\abs{\abs\var}}{\abs{\app{\abs\var}\var}}
}


==> figs/pstricks/lambdatgs_over_siglambda12_not_closed_under_funcbisim_eager.tex <==
\lgr
{
\app{\abs{\s{{\abs\var}}}}{\abs{\app{\s{\abs\var}}\var}}
}


==> figs/pstricks/macros/lambdagraph.tex <==
% Named Lambda Graph with Invisible Scopes

\newcommand\tree[2]{\pstree[linewidth=0.5pt,nodesep=0.4mm,levelsep=0.8cm]{#1}{#2}}
\newcommand\node[1]{\TR{#1}}

% The Language

\newcommand\lgr[1]{\ensuremath{\tree{\nil}{#1}}}

\newcommand\abs[1]{\tree{\node{\lambda}}{#1}}
\newcommand\s[1]{\tree{\node S}{#1}}
\newcommand\app[2]{\tree{\node{@}}{#1 #2}}
\newcommand\var{\tree{\node{0}}{\nil}}

\newcommand\labs[3]{\tree{\node{\lambda_{#1}^{\small(#2\small)}}}{#3}}
\newcommand\ls[2]{\tree{\node{S^{(#1)}}}{#2}}
\newcommand\lapp[3]{\tree{\node{@^{(#1)}}}{#2 #3}}
\newcommand\lvar[1]{\tree{\node{0^{(#1)}}}{\nil}}

\newcommand\etc[0]{\node{\vdots}}
\newcommand\op[1]{\Tcircle{#1}}
\newcommand\nil{\node{}}


==> figs/pstricks/macros/ltg-bl.tex <==
% Lambda Transition Graph with Back-Links

% CAUTION: The lambda-letrec constructors are supposed to be used as unsaturated functions.
%          The last two parameters are all supplied here.
%          First paramater: labelling of the incoming edge
%          Second paramater: labelling of this node

\newcommand\mkNode\Toval
\newcommand\putEdge{\mput*}
\newcommand\tree[2]{\pstree[arrows=->,treesep=1cm,levelsep=1.5cm]{#1}{#2}}
\newcommand\node[1]{\mkNode{\nlabel{#1}}}


% The Language

%\newcommand\lambdaterm[1]{\ensuremath{\tree{\TR{}}{#1{}{}}}}
\newcommand\lambdaterm[1]{\ensuremath{#1{}{}}}

\newcommand\app[4]{\tree{\node{#4}#3}{#1{\putEdge{@_0}}{#4} #2{\putEdge{@_1}}{#4}}}

\newcommand\abs[4]{\tree{\rnode{#1}{\node{#4}}#3}{#2{\putEdge\lambda}{#4#1}}}

\newcommand\s[3]{
	\StrGobbleRight{#3}1[\NewStr]
	\tree{\node{#3}#2}{#1{\putEdge S}\NewStr}
}

\newcommand\sA[3]{
	\StrGobbleRight{#3}1[\NewStri]
	\tree{\node{#3}#2}{#1{\putEdge S}\NewStri}
}

\newcommand\sapp[5]{
	\StrGobbleRight{#5}1[\NewStri]
	\tree{\node{#5}#4}{#1{\putEdge S}\NewStri #2{\putEdge{@_0}}{#5} #3{\putEdge{@_1}}{#5}}
}

\newcommand\cprapp[6]{
	\StrDel[1]{#6}{#1}[\ANewStrin]
	\tree{\node{#6}#5}{#2{\putEdge{del}}\ANewStrin #3{\putEdge{@_0}}{#6} #4{\putEdge{@_1}}{#6}}
}

\newcommand\cpr[4]{
	\StrDel[1]{#4}{#1}[\NewStrin]
	\tree{\node{#4}#3}{#2{\putEdge{del}}\NewStrin}
}

\newcommand\cpR[4]{
	\StrDel[1]{#4}{#1}[\NewString]
	\tree{\node{#4}#3}{#2{\putEdge{del}}\NewString}
}

\newcommand\var[3]{{\psset{nodesepB=0pt}\mkNode[name=here]{\nlabel{#3}}#2}\ncangles[nodesepA=0pt]{->}{here}{#1}\ncput*{0}}
\newcommand\vara[5]{{\psset{nodesepB=0pt}\mkNode[name=here]{\nlabel{#5}}#4}\ncangles[nodesepA=0pt,angleA=#2,angleB=#3]{->}{here}{#1}\ncput*{0}}

\newcommand\etc[2]{\TR{\vdots}#1}

\newcommand\letbind[4]{#2{\rnode{#1}{}#3}{#4}}

\newcommand\letvar[3]{{\psset{arrows=-,nodesepB=0pt}\Tp*[name=here]}\ncangles[angleB=70,nodesepA=0pt]{->}{here}{#1}#2}
\newcommand\letvara[5]{{\psset{arrows=-,nodesepB=0pt}\Tp*[name=here]}\ncangles[angleA=#2,angleB=#3,nodesepA=0pt]{->}{here}{#1}#4}

%\newcommand\op[3]{\tree{\node{#3}#2}{\mkNode{#1}}}
%\newcommand\op[3]{\var{#1}{#2}{#3}}
%\newcommand\op[3]{\etc{#2}{#3}}
\newcommand\op[3]{\TR{\dots}#2}

\newcommand\nil[2]{\node{#2}#1}


==> figs/pstricks/macros/ltg.tex <==
% The Lambda Transition Graph without Back-Links

\input{macros/ltg-bl}

\renewcommand\var[3]{\tree{\node{#3}#2}{}}
\renewcommand\vara[5]{\tree{\node{#5}#4}{}}


==> figs/pstricks/macros/scopedgraph.tex <==
% Nameless Lambda Graph with Visible Scopes

\input{macros/lambdagraph}

\renewcommand\abs[2]{\tree{\node{\lambda}}{#2}}
\renewcommand\s[1]{\tree{\node S}{#1}}
\renewcommand\var[1]{\node{0}}
\renewcommand\vara[3]{\node{0}}


==> figs/pstricks/mk/postlude.tex <==
\end{document}


==> figs/pstricks/no_extension_funbisim_siglambda1_g0.tex <==
\lgr{
\abs{\app{\nil}{\app\var\var}}
}


==> figs/pstricks/no_extension_funbisim_siglambda1_g1.tex <==
\lgr{
\abs{\app{\abs{\app{\nil}{\app\var\var}}}{\app\var\var}}
}


==> figs/pstricks/rem_corr_laphotgs_ltgs_nobij_aphotg.tex <==
\lgr{
\labs{v_1}{}{\lapp{v_1}{\labs{v_2}{v_1}{\lvar{v_1}}}{\labs{v_3}{v_1}\nil}}
}


==> figs/pstricks/rem_corr_laphotgs_ltgs_nobij_snodes.tex <==
\lgr{
\abs{\app{\abs{\s\var}}{\abs\nil}}
}


==> figs/pstricks/running_ho_tg.tex <==
\lgr{
\abs{\app{\abs{\app\var{{\app\var{{\abs\var}}}}}}{{\abs{{{\app\nil\nil}}}}}}
}


==> figs/pstricks/running_prefixed_ho_tg_eager.tex <==
\lgr{
\labs{v_0}{}{\lapp{v_0}{\labs{v_1}{v_0}{\lapp{v_0v_1}{\lvar{v_0v_1}}{{\lapp{v_0}{\lvar{v_0}}{{\labs{v_2}{}{\lvar{v_2}}}}}}}}{{\labs{v_3}{}{{{\lapp{}\nil\nil}}}}}}
}


==> figs/pstricks/running_prefixed_ho_tg_non_eager.tex <==
\lgr{
\labs{v_0}{}{\lapp{v_0}{\labs{v_1}{v_0}{\lapp{v_0v_1}{\lvar{v_0v_1}}{\lapp{v_0v_1}{\lvar{v_0}}{{\labs{v_2}{}{\lvar{v_2}}}}}}}{\labs{v_3}{v_0}{{{\lapp{v_0}\nil\nil}}}}}
}


==> figs/pstricks/running_snodes_eager.tex <==
\lgr{
\abs{\app{\abs{\app\var{\s{\app\var{\s{\abs\var}}}}}}{\s{\abs{\s{{\app\nil\nil}}}}}}
}


==> figs/pstricks/running_snodes_non_eager.tex <==
\lgr{
\abs{\app{\abs{\app\var{\app{\s\var}{\s{\s{\abs\var}}}}}}{\abs{\s{\app{\s\nil}{\s\nil}}}}}
}

